InteractDiffusion: Interaction Control in Text-to-Image Diffusion Models

Large-scale text-to-image (T2I) diffusion models have showcased incredible capabilities in generating coherent images based on textual descriptions, enabling vast applications in content generation. While recent advancements have introduced control over factors such as object localization, posture, and image contours, a crucial gap remains in our ability to control the interactions between objects in the generated content. Well-controlling interactions in generated images could yield meaningful applications, such as creating realistic scenes with interacting characters. In this work, we study the problems of conditioning T2I diffusion models with Human-Object Interaction (HOI) information, consisting of a triplet label (person, action, object) and corresponding bounding boxes. We propose a pluggable interaction control model, called InteractDiffusion that extends existing pre-trained T2I diffusion models to enable them being better conditioned on interactions. Specifically, we tokenize the HOI information and learn their relationships via interaction embeddings. A conditioning self-attention layer is trained to map HOI tokens to visual tokens, thereby conditioning the visual tokens better in existing T2I diffusion models. Our model attains the ability to control the interaction and location on existing T2I diffusion models, which outperforms existing baselines by a large margin in HOI detection score, as well as fidelity in FID and KID. Project page: https://jiuntian.github.io/interactdiffusion.

==> assets/figure/diff2_object.tex <==

\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{0.5pt} % General space between cols (6pt standard)
    \renewcommand{\arraystretch}{1} % General space between rows (1 standard)
    \begin{tabular}{ccccccc}
       % \toprule
        % & & a & b & c & d \\
        % \midrule
        \raisebox{-0.15\height}{\frame{\includegraphics[width=.23\linewidth]{assets/images/diff_object/x1y1.png}}}
        & \raisebox{-0.15\height}{\includegraphics[width=.23\linewidth]{assets/images/diff_object/x2y1.png}}
        & \raisebox{-0.15\height}{\includegraphics[width=.23\linewidth]{assets/images/diff_object/x3y1.png}}
        & \raisebox{-0.15\height}{\includegraphics[width=.23\linewidth]{assets/images/diff_object/x5y1.png}}
        \\
        \footnotesize a girl is holding a \textlangle*\textrangle
        & hamburger
        & book
        & toy car
    \end{tabular}
    \captionsetup{type=figure}
    \caption{Visualization comparison between InteractDiffusion StableDiffusion and GLIGEN* demonstrating the generation of {\it different objects} for the same action.}
    \label{fig:diff_object2}
    \vspace{-10pt}
\end{table}

==> assets/figure/tab_ablation.tex <==
\begin{table}[t]
\centering
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\setlength{\tabcolsep}{3pt} % General space between cols (6pt standard)
\resizebox{8cm}{!}{
\begin{tabular}{l|lll|cc|cc|cc}
\hline
\multirow{2}{*}{Model}             & \multirow{2}{*}{Tr.} & \multirow{2}{*}{To.} & \multirow{2}{*}{Em.} & \multicolumn{2}{l|}{Quality}        & \multicolumn{2}{l|}{Default~$\uparrow$} & \multicolumn{2}{l}{Known Object~$\uparrow$} \\ \cline{5-10} 
                                   &                      &                      &                      & FID~$\downarrow$ & KID~$\downarrow$ & Full               & Rare               & Full                 & Rare                 \\ \hline
StableDiffusion               &                      &                      &                      & 35.85            & 0.01297          & 0.63               & 0.68               & 0.66                 & 0.70                 \\
GLIGEN                             & \checkmark *         &                      &                      & 28.97            & 0.01216          & 21.73              & 15.35              & 23.31                & 17.24                \\
GLIGEN*                            & \checkmark *         &                      &                      & 18.82            & 0.00694          & 25.23              & 17.45              & 26.66                & 18.78                \\
\multirow{2}{*}{InteractDiffusion} & \checkmark           & \checkmark           &                      & 18.88            & 0.00686          & 28.73              & 21.93              & 30.15                & 23.38                \\
                                   & \checkmark           & \checkmark           & \checkmark           & \textbf{18.69}   & \textbf{0.00676} & \textbf{29.53}     & \textbf{23.02}     & \textbf{30.99}       & \textbf{24.93}       \\ \hline
HICO-DET                           &                      &                      &                      & -                & -                & 29.94              & 22.24              & 32.48                & 24.16                \\ \hline
\end{tabular}}
\caption{Ablation study of various key components in our InteractDiffusion. GLIGEN* is HICO-DET fine-tuned GLIGEN model. Tr., To., and Em. represents Interaction Transformer, Interaction Tokenizer, and Interaction Embedding respectively. \checkmark* indicate Gated Self-Attention in GLIGEN. \textbf{Bold} values indicate best performance in the column.}
\label{tab:ablation}
\end{table}

==> assets/figure/tab_performance.tex <==
\begin{table*}[t]
\centering
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\setlength{\tabcolsep}{3pt} % General space between cols (6pt standard)
\resizebox{12cm}{!}{
\begin{tabular}{l|ll|cccc|cccc}
\hline
\multirow{3}{*}{Model} & \multicolumn{2}{l|}{\multirow{2}{*}{Quality}}                                & \multicolumn{4}{c|}{Tiny}                                                                           & \multicolumn{4}{c}{Large}                                                                          \\ \cline{4-11} 
                       & \multicolumn{2}{l|}{}                                                        & \multicolumn{2}{l|}{Default~$\uparrow$}              & \multicolumn{2}{l|}{Known Object~$\uparrow$} & \multicolumn{2}{c|}{Default~$\uparrow$}              & \multicolumn{2}{l}{Known Object~$\uparrow$} \\ \cline{2-11} 
                       & \multicolumn{1}{c}{FID~$\downarrow$} & \multicolumn{1}{c|}{KID~$\downarrow$} & Full           & \multicolumn{1}{c|}{Rare}           & Full                  & Rare                 & Full           & \multicolumn{1}{c|}{Rare}           & Full                 & Rare                 \\ \hline
StableDiffusion   & 35.85                                & 0.01297                               & 0.63           & \multicolumn{1}{c|}{0.68}           & 0.66                  & 0.70                 & 0.64           & \multicolumn{1}{c|}{0.83}           & 0.65                 & 0.84                 \\
GLIGEN                 & 29.35                                & 0.01275                               & 21.73          & \multicolumn{1}{c|}{15.35}          & 23.31                 & 17.24                & 23.99          & \multicolumn{1}{c|}{19.56}          & 24.99                & 20.37                \\
GLIGEN*                & 18.82                                & 0.00694                               & 25.23          & \multicolumn{1}{c|}{17.45}          & 26.66                 & 18.78                & 26.45          & \multicolumn{1}{c|}{18.93}          & 27.32                & 19.90                \\
InteractDiffusion      & \textbf{18.73}                       & \textbf{0.00668}                      & \textbf{29.53} & \multicolumn{1}{c|}{\textbf{23.02}} & \textbf{30.99}        & \textbf{24.93}       & \textbf{31.56} & \multicolumn{1}{c|}{\textbf{26.09}} & \textbf{32.52}       & \textbf{27.04}       \\ \hline
HICO-DET               & \multicolumn{1}{c}{-}                & \multicolumn{1}{c|}{-}                & 29.94          & \multicolumn{1}{c|}{22.24}          & 32.48                 & 24.16                & 37.18          & \multicolumn{1}{c|}{30.71}          & 38.93                & 31.93                \\ \hline
\end{tabular}}
\caption{Performance of our InteractDiffusion compared to existing baselines in term of quality and HOI detection score. Quality column shows the quality of the generated image, the lower is better. HOI Detection Score is obtained using FGAHOI and is measured in mean average precision (mAP), using Swin-Tiny and Swin-Large backbone, which indicate the controllability toward the interaction in the image generation, the higher of which is better. GLIGEN* is HICO-DET fine-tuned GLIGEN model. \textbf{Bold} values indicate best performance in the column. The last row shows the Detection Score from real images.}
\label{tab:fid_map}
\end{table*}
